Uncertainty in Multi-Commodity Routing Networks: When does it help?

We study the equilibrium behavior in a multi-commodity selfish routing game with many types of uncertain users where each user over- or under-estimates their congestion costs by a multiplicative factor. Surprisingly, we find that uncertainties in different directions have qualitatively distinct impacts on equilibria. Namely, contrary to the usual notion that uncertainty increases inefficiencies, network congestion actually decreases when users over-estimate their costs. On the other hand, under-estimation of costs leads to increased congestion. We apply these results to urban transportation networks, where drivers have different estimates about the cost of congestion. In light of the dynamic pricing policies aimed at tackling congestion, our results indicate that users' perception of these prices can significantly impact the policy's efficacy, and "caution in the face of uncertainty" leads to favorable network conditions.

==> illustrativeex.tex <==

%\subsection{Illustrative Example: Parking and Through--Traffic Users}
\begin{figure}[t!]
	\centering
	\begin{tikzpicture}
	\begin{scope}

	\node (fr) at (0, -0.4) {};

	\begin{scope}%[scale=1.2]
	\node (arbit1) at (1.5, 0.5) {};
	\node (arbit2) at (1.5, -1.8) {};
%	\draw (fr) +(0, -0.2) node[normalNodeS] (s1) {};
		\draw (fr) +(-1, -1.0) node[labeledNodeS] (org){$s$};
	\draw (fr) +(5 ,-0.5) node[labeledNodeS] (v1) {$t_{\type_1}$}
	edge[normalEdgeF, <-,bend right] node[above] {$e_1$} (org) ;

%	edge[normalEdgeF, <-] node[below] {} (s1) ;
	%edge[normalEdgeF, <-] node[left] {$0$} (v1);
%	\draw (fr) +(3, 0) node[normalNodeS] (t1) {};
%	edge[normalEdgeF, <-] node[above] {} (v1)
%	edge[normalEdgeF, <-] node[below] {} (v2);

%	edge[normalEdgeF, ->] node[below] {} (s1) ;


	\draw (fr) +(2.2,-1)  node[labeledNodeS] (dest){$i$}
	edge[normalEdgeF, ->] node[above] {$e_3$} (v1) {}
		edge[normalEdgeF, <-] node[below] {$e_2$} (org);
%	edge[normalEdgeF, <-] node[above] {} (mid);


	\draw (fr) +(5,-1.5)  node[labeledNodeS] (dest2){$t_{\type_2}$}
		edge[normalEdgeF, <-] node[below] {$e_4$} (dest)
		edge[normalEdgeF, <-, bend left] node[below] {$e_5$} (org);
	%edge[normalEdgeF, <-] node[above] {$e_4$} (mid)

%	\draw(fr) +(2,-3) node[normalNodeS] (pg){G}
%	edge[normalEdgeF, <-,bend left] node[right] {Parking Space 1} (mid);

%	\node (arbit3) at (1.6, -0.5) [draw,rotate=290,inner sep = 1] {\footnotesize Parking $1$};
	%	\node (arbit3) at (1.6, -2.1) [draw,rotate=65,inner sep=1] {\footnotesize Parking $2$};
	%		\node (arbit3) at (5.4, -2.5) [text width = 1.7cm] {\footnotesize Destination for type $\theta_2$};
%			\node (arbit4) at (5.2, 0) [text width = 1.7cm] {\footnotesize Destination for type $\theta_1$};
	\end{scope}

	\end{scope}
	\end{tikzpicture}
	\caption{\label{fig:parkingroutingbasic} An abstract example of a two-commodity routing game, where all traffic originates at node $s$. Users of type $\type_1$ select a route between nodes $s$ and $t_{\type_1}$, whereas users of type $\type_2$ route traffic between $s$ and $t_{\type_2}$. }

\end{figure}

\subsection{Illustrative Example }
\todo{Make this example more general by deleting stuff about transportation. The message is a little bit lost here. Figure 1 occurs in many application anyways, so just describe what happens where there is uncertainty. Also makes the discussion shorter.}
%\lily{if you cant keep the title to one line, then its too long}
%%%%%% OLD Example %%%%%%
%%\lily{if you cant keep the title to one line, then its too long}
%To get a better feel for our multi-commodity routing model, let us consider the example depicted Fig.~\ref{fig:parkingroutingbasic} of a simple network that
%captures the conflict between two types of users. Such a situation could occur
%in a number of applications pertaining to urban transportation where different
%types of users compete for the same resources. For concreteness, suppose that
%$\type_1$ represents travelers who choose between public transportation or
%ride-sharing (path $\{e_2, e_3\}$) and simply walking to their final
%destination (edge $e_1$). On the other hand, $\type_2$ could denote drivers with
%personal vehicles (paths $\{e_2,e_4\}$ and $\{e_5\}$).
%%\lily{I am a little confused by this example since there are more paths than
%%described}
%
%
%Suppose that $C_{e_2}(x) = ax$ for some parameter $a > 0$---this captures the
%congestion costs faced both by users of type $\type_1$ (on a vehicle) and users
%of type $\type_2$.  Users on edge $e_1$ experience costs associated with
%walking, whereas users on edge $e_3$ experience  (e.g.,) the delays involved in
%public transportation or the price of ride-sharing. Due to the proliferation of
%global positioning systems (GPS), it is reasonable to assume that users of type
%$\type_2$ have no uncertainty ($r_{\type_2} = 1$). On the contrary, users of type $\type_1$ could be averse to (or even favor) walking long distances and therefore $r_{\type_1} \neq 1$.
%
%
%
%To illustrate the behavior of users with uncertainty, observe that when
%$r_{\type_1} > 1$, more users of type $\type_1$ would select the direct edge
%$e_1$ (to avoid congestion on uncertain edges) leading to faster travel times
%for users of type $\type_1$. When these users prefer $e_2$ (e.g., when
%$r_{\type_1} < 1$ ), this leads to increased congestion for the driving users
%forcing more users to switch to $e_5$. While this instance was described only
%for illustrative purposes, user behavior under uncertainty for more realistic
%and nuanced examples can be seen in Section~\ref{sec:simulations} for
%transportation networks where users searching for parking compete with through
%traffic.
%%%%%% END OLd Example



To get a better feel for our multi-commodity routing model, let us consider the example depicted Fig.~\ref{fig:parkingroutingbasic} of a simple network that
captures the conflict between two types of users. 

%Such a situation could occur
%in a number of applications pertaining to urban transportation where different
%types of users compete for the same resources. 
%For concreteness, suppose that
%$\type_1$ represents users who choose between public transportation or
%ride-sharing (path $\{e_2, e_3\}$) and simply walking to their final
%destination (edge $e_1$). On the other hand, $\type_2$ could denote drivers with
%personal vehicles (paths $\{e_2,e_4\}$ and $\{e_5\}$).
%\lily{I am a little confused by this example since there are more paths than
%described}

Suppose that $C_{e_2}(x) = ax$ for some parameter $a > 0$---this captures the
congestion costs faced both by users of type $\type_1$  and users
of type $\type_2$. Further, assume that type $\type_1$ users are uncertain with
$r_{\type_1} \neq 1$ and type $\type_2$ users are certain---i.e.~$r_{\type_2} =
1$. 
%Users on edge $e_1$ experience costs associated with
%walking, whereas users on edge $e_3$ experience  (e.g.,) the delays involved in
%public transportation or the price of ride-sharing. Due to the proliferation of
%global positioning systems (GPS), it is reasonable to assume that users of type
%Assume that users of type $\type_2$ have no uncertainty ($r_{\type_2} = 1$) and users of type $\type_1$ 
%%could be averse to (or even favor) walking long distances and therefore
%have uncertainty $r_{\type_1} \neq 1$.

To illustrate the behavior of users with uncertainty, observe that when $r_{\type_1} > 1$, more users of type $\type_1$
select the direct edge $e_1$ (to avoid congestion on uncertain edges
\textcolor{red}{arent all edges uncertain for this user type including $e_1$?
Perhaps the example isnt clear\ldots are you just considering constant costs on
all the other edges?}
).
%leading to
%lower congestion costs. 
When $r_{\type_1} < 1$, type $\type_1$ users prefer $e_2$ and this leads to
increased congestion users of type $\type_2$ forcing more users to switch to $e_5$. While this instance was described only for illustrative purposes, user behavior under uncertainty for more realistic and nuanced examples can be seen in Section~\ref{sec:simulations} for transportation networks where users searching for parking compete with through traffic.
\textcolor{red}{I actually dont think this example is illustrative. What is the
    point or message? That users switch choices when there are different costs,
well that is obvious\ldots What are we trying to illustrate with this example? I
also think if we are going to have a illustrative example it has to come after
we define how users choose paths not before! My suggestion is we should remove
this example. It will buy us space and we dont lose anythign interesting.}


